Bias amplification in experimental social networks is reduced by resampling

Large-scale social networks are thought to contribute to polarization by amplifying people's biases. However, the complexity of these technologies makes it difficult to identify the mechanisms responsible and to evaluate mitigation strategies. Here we show under controlled laboratory conditions that information transmission through social networks amplifies motivational biases on a simple perceptual decision-making task. Participants in a large behavioral experiment showed increased rates of biased decision-making when part of a social network relative to asocial participants, across 40 independently evolving populations. Drawing on techniques from machine learning and Bayesian statistics, we identify a simple adjustment to content-selection algorithms that is predicted to mitigate bias amplification. This algorithm generates a sample of perspectives from within an individual's network that is more representative of the population as a whole. In a second large experiment, this strategy reduced bias amplification while maintaining the benefits of information sharing.

==> stats/e1/tests/chose_bias/aso_bias-soc_bias/prereg.tex <==
$\chi^2(1)=29.85$, $p<0.001$


==> stats/e1/tests/chose_bias/aso_bias-soc_control/prereg.tex <==
$\chi^2(1)=22.29$, $p<0.001$


==> stats/e1/tests/chose_bias/aso_control-aso_bias/prereg.tex <==
$\chi^2(1)=12.68$, $p<0.001$


==> stats/e1/tests/chose_bias/aso_control-soc_bias/prereg.tex <==
$\chi^2(1)=78.48$, $p<0.001$


==> stats/e1/tests/chose_bias/aso_control-soc_bias/reported.tex <==
$\chi^2(1)=83.44$, $p<0.001$


==> stats/e1/tests/chose_bias/aso_control-soc_control/prereg.tex <==
$\chi^2(1)=1.65$, $p=0.198$


==> stats/e1/tests/chose_bias/aso_control-soc_control/reported.tex <==
$\chi^2(1)=1.74$, $p=0.187$


==> stats/e1/tests/chose_bias/soc_bias-soc_control/prereg.tex <==
$\chi^2(1)=96.03$, $p<0.001$


==> stats/e1/tests/chose_bias/soc_bias-soc_control/reported.tex <==
$\chi^2(1)=102.45$, $p<0.001$


==> stats/e1/tests/chose_correct/aso_bias-soc_bias/prereg.tex <==
$\chi^2(1)=15.07$, $p<0.001$


==> stats/e1/tests/chose_correct/aso_bias-soc_control/prereg.tex <==
$\chi^2(1)=22.58$, $p<0.001$


==> stats/e1/tests/chose_correct/aso_control-aso_bias/prereg.tex <==
$\chi^2(1)=0.1$, $p=0.746$


==> stats/e1/tests/chose_correct/aso_control-aso_bias/reported.tex <==
$\chi^2(1)=0.1$, $p=0.746$


==> stats/e1/tests/chose_correct/aso_control-soc_bias/prereg.tex <==
$\chi^2(1)=17.6$, $p<0.001$


==> stats/e1/tests/chose_correct/aso_control-soc_control/prereg.tex <==
$\chi^2(1)=25.65$, $p<0.001$


==> stats/e1/tests/chose_correct/soc_bias-soc_control/prereg.tex <==
$\chi^2(1)=0.71$, $p=0.399$


==> stats/e1/tests/chose_correct/soc_bias-soc_control/reported.tex <==
$\chi^2(1)=0.71$, $p=0.399$


==> stats/e1_exploratory/matched/means/chose_bias/aso_bias/percentage.tex <==
67


==> stats/e1_exploratory/matched/means/chose_bias/aso_bias/proportion.tex <==
0.67


==> stats/e1_exploratory/matched/means/chose_bias/aso_control/percentage.tex <==
63


==> stats/e1_exploratory/matched/means/chose_bias/aso_control/proportion.tex <==
0.63


==> stats/e1_exploratory/matched/means/chose_bias/soc_bias/percentage.tex <==
76.4


==> stats/e1_exploratory/matched/means/chose_bias/soc_bias/proportion.tex <==
0.764


==> stats/e1_exploratory/matched/means/chose_bias/soc_control/percentage.tex <==
66.7


==> stats/e1_exploratory/matched/means/chose_bias/soc_control/proportion.tex <==
0.667


==> stats/e1_exploratory/matched/means/chose_correct/aso_bias/proportion.tex <==
0.67


==> stats/e1_exploratory/matched/means/chose_correct/aso_control/proportion.tex <==
0.63


==> stats/e1_exploratory/matched/means/chose_correct/soc_bias/proportion.tex <==
0.764


==> stats/e1_exploratory/matched/means/chose_correct/soc_control/proportion.tex <==
0.667


==> stats/e1_exploratory/matched/tests/chose_bias/aso_bias-soc_bias/prereg.tex <==
$\chi^2(1)=49.87$, $p<0.001$


==> stats/e1_exploratory/matched/tests/chose_bias/aso_bias-soc_bias/reported.tex <==
$\chi^2(1)=53.28$, $p<0.001$


==> stats/e1_exploratory/matched/tests/chose_bias/aso_bias-soc_control/prereg.tex <==
$\chi^2(1)=0.03$, $p=0.859$


==> stats/e1_exploratory/matched/tests/chose_bias/aso_bias-soc_control/reported.tex <==
$\chi^2(1)=0.04$, $p=0.85$


==> stats/e1_exploratory/matched/tests/chose_bias/aso_control-aso_bias/prereg.tex <==
$\chi^2(1)=8.11$, $p=0.004$


==> stats/e1_exploratory/matched/tests/chose_bias/aso_control-aso_bias/reported.tex <==
$\chi^2(1)=8.65$, $p=0.003$


==> stats/e1_exploratory/matched/tests/chose_bias/aso_control-soc_bias/prereg.tex <==
$\chi^2(1)=95.37$, $p<0.001$


==> stats/e1_exploratory/matched/tests/chose_bias/aso_control-soc_bias/reported.tex <==
$\chi^2(1)=102.43$, $p<0.001$


==> stats/e1_exploratory/matched/tests/chose_bias/aso_control-soc_control/prereg.tex <==
$\chi^2(1)=6.62$, $p=0.01$


==> stats/e1_exploratory/matched/tests/chose_bias/aso_control-soc_control/reported.tex <==
$\chi^2(1)=7.03$, $p=0.008$


==> stats/e1_exploratory/matched/tests/chose_bias/soc_bias-soc_control/prereg.tex <==
$\chi^2(1)=49.2$, $p<0.001$


==> stats/e1_exploratory/matched/tests/chose_bias/soc_bias-soc_control/reported.tex <==
$\chi^2(1)=52.68$, $p<0.001$


==> stats/e1_exploratory/matched/tests/chose_correct/aso_bias-soc_bias/prereg.tex <==
$\chi^2(1)=49.87$, $p<0.001$


==> stats/e1_exploratory/matched/tests/chose_correct/aso_bias-soc_control/prereg.tex <==
$\chi^2(1)=0.03$, $p=0.859$


==> stats/e1_exploratory/matched/tests/chose_correct/aso_bias-soc_control/reported.tex <==
$\chi^2(1)=0.04$, $p=0.85$


==> stats/e1_exploratory/matched/tests/chose_correct/aso_control-aso_bias/prereg.tex <==
$\chi^2(1)=8.11$, $p=0.004$


==> stats/e1_exploratory/matched/tests/chose_correct/aso_control-aso_bias/reported.tex <==
$\chi^2(1)=8.65$, $p=0.003$


==> stats/e1_exploratory/matched/tests/chose_correct/aso_control-soc_bias/prereg.tex <==
$\chi^2(1)=95.37$, $p<0.001$


==> stats/e1_exploratory/matched/tests/chose_correct/aso_control-soc_bias/reported.tex <==
$\chi^2(1)=102.43$, $p<0.001$


==> stats/e1_exploratory/matched/tests/chose_correct/aso_control-soc_control/prereg.tex <==
$\chi^2(1)=6.62$, $p=0.01$


==> stats/e1_exploratory/matched/tests/chose_correct/soc_bias-soc_control/prereg.tex <==
$\chi^2(1)=49.2$, $p<0.001$


==> stats/e1_exploratory/matched/tests/chose_correct/soc_bias-soc_control/reported.tex <==
$\chi^2(1)=52.68$, $p<0.001$


==> stats/e1_exploratory/nonmatched/means/chose_bias/aso_bias/percentage.tex <==
45.4


==> stats/e1_exploratory/nonmatched/means/chose_bias/aso_bias/proportion.tex <==
0.454


==> stats/e1_exploratory/nonmatched/means/chose_bias/aso_control/percentage.tex <==
42.1


==> stats/e1_exploratory/nonmatched/means/chose_bias/aso_control/proportion.tex <==
0.421


==> stats/e1_exploratory/nonmatched/means/chose_bias/soc_bias/percentage.tex <==
47.2


==> stats/e1_exploratory/nonmatched/means/chose_bias/soc_bias/proportion.tex <==
0.472


==> stats/e1_exploratory/nonmatched/means/chose_bias/soc_control/percentage.tex <==
35.8


==> stats/e1_exploratory/nonmatched/means/chose_bias/soc_control/proportion.tex <==
0.358


==> stats/e1_exploratory/nonmatched/means/chose_correct/aso_bias/proportion.tex <==
0.546


==> stats/e1_exploratory/nonmatched/means/chose_correct/aso_control/proportion.tex <==
0.579


==> stats/e1_exploratory/nonmatched/means/chose_correct/soc_bias/proportion.tex <==
0.528


==> stats/e1_exploratory/nonmatched/means/chose_correct/soc_control/proportion.tex <==
0.642


==> stats/e1_exploratory/nonmatched/tests/chose_bias/aso_bias-soc_bias/prereg.tex <==
$\chi^2(1)=1.53$, $p=0.216$


==> stats/e1_exploratory/nonmatched/tests/chose_bias/aso_bias-soc_bias/reported.tex <==
$\chi^2(1)=1.57$, $p=0.211$


==> stats/e1_exploratory/nonmatched/tests/chose_bias/aso_bias-soc_control/prereg.tex <==
$\chi^2(1)=44.83$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_bias/aso_bias-soc_control/reported.tex <==
$\chi^2(1)=46.06$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_bias/aso_control-aso_bias/prereg.tex <==
$\chi^2(1)=5.49$, $p=0.019$


==> stats/e1_exploratory/nonmatched/tests/chose_bias/aso_control-aso_bias/reported.tex <==
$\chi^2(1)=5.61$, $p=0.018$


==> stats/e1_exploratory/nonmatched/tests/chose_bias/aso_control-soc_bias/prereg.tex <==
$\chi^2(1)=12.23$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_bias/aso_control-soc_bias/reported.tex <==
$\chi^2(1)=12.53$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_bias/aso_control-soc_control/prereg.tex <==
$\chi^2(1)=19.79$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_bias/aso_control-soc_control/reported.tex <==
$\chi^2(1)=20.28$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_bias/soc_bias-soc_control/prereg.tex <==
$\chi^2(1)=58.81$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_bias/soc_bias-soc_control/reported.tex <==
$\chi^2(1)=60.56$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_correct/aso_bias-soc_bias/prereg.tex <==
$\chi^2(1)=1.53$, $p=0.216$


==> stats/e1_exploratory/nonmatched/tests/chose_correct/aso_bias-soc_control/prereg.tex <==
$\chi^2(1)=44.83$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_correct/aso_bias-soc_control/reported.tex <==
$\chi^2(1)=46.06$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_correct/aso_control-aso_bias/prereg.tex <==
$\chi^2(1)=5.49$, $p=0.019$


==> stats/e1_exploratory/nonmatched/tests/chose_correct/aso_control-aso_bias/reported.tex <==
$\chi^2(1)=5.61$, $p=0.018$


==> stats/e1_exploratory/nonmatched/tests/chose_correct/aso_control-soc_bias/prereg.tex <==
$\chi^2(1)=12.23$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_correct/aso_control-soc_bias/reported.tex <==
$\chi^2(1)=12.53$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_correct/aso_control-soc_control/prereg.tex <==
$\chi^2(1)=19.79$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_correct/soc_bias-soc_control/prereg.tex <==
$\chi^2(1)=58.81$, $p<0.001$


==> stats/e1_exploratory/nonmatched/tests/chose_correct/soc_bias-soc_control/reported.tex <==
$\chi^2(1)=60.56$, $p<0.001$


==> stats/e1_perceptual_priming/summaries/chose_green/percentage.tex <==
53.5


==> stats/e1_perceptual_priming/summaries/green_shown=FALSE/chose_green/percentage.tex <==
52.3


==> stats/e1_perceptual_priming/summaries/green_shown=FALSE/n.tex <==
384


==> stats/e1_perceptual_priming/summaries/green_shown=TRUE/chose_green/percentage.tex <==
54.7


==> stats/e1_perceptual_priming/summaries/green_shown=TRUE/n.tex <==
408


==> stats/e1_perceptual_priming/summaries/randomization_color=blue/chose_green/percentage.tex <==
47.5


==> stats/e1_perceptual_priming/summaries/randomization_color=blue/n.tex <==
396


==> stats/e1_perceptual_priming/summaries/randomization_color=green/chose_green/percentage.tex <==
59.6


==> stats/e1_perceptual_priming/summaries/randomization_color=green/n.tex <==
396


==> stats/e2/tests/chose_bias/aso_bias-soc_bias/prereg.tex <==
$\chi^2(1)=7.63$, $p=0.006$


==> stats/e2/tests/chose_bias/aso_bias-soc_resampling/prereg.tex <==
$\chi^2(1)=3.79$, $p=0.052$


==> stats/e2/tests/chose_bias/aso_bias-soc_resampling/reported.tex <==
$\chi^2(1)=0.5$, $p=0.477$


==> stats/e2/tests/chose_bias/soc_resampling-soc_bias/prereg.tex <==
$\chi^2(1)=11.29$, $p<0.001$


==> stats/e2/tests/chose_correct/aso_bias-soc_bias/prereg.tex <==
$\chi^2(1)=26.07$, $p<0.001$


==> stats/e2/tests/chose_correct/aso_bias-soc_resampling/prereg.tex <==
$\chi^2(1)=10.49$, $p=0.001$


==> stats/e2/tests/chose_correct/soc_resampling-soc_bias/prereg.tex <==
$\chi^2(1)=1.89$, $p=0.17$


==> stats/e2_exploratory/means/social_info_accuracy/soc_bias/proportion.tex <==
0.623


==> stats/e2_exploratory/means/social_info_accuracy/soc_resampling/proportion.tex <==
0.64


==> stats/e2_exploratory/means/social_info_bias/soc_bias/proportion.tex <==
0.564


==> stats/e2_exploratory/means/social_info_bias/soc_resampling/proportion.tex <==
0.508


==> stats/e2_exploratory/means/social_info_green/social_bias/blue_bias/percentage.tex <==
51.9


==> stats/e2_exploratory/means/social_info_green/social_bias/blue_bias/proportion.tex <==
0.519


==> stats/e2_exploratory/means/social_info_green/social_bias/green_bias/percentage.tex <==
64.6


==> stats/e2_exploratory/means/social_info_green/social_bias/green_bias/proportion.tex <==
0.646


==> stats/e2_exploratory/means/social_info_green/social_resampling/blue_bias/percentage.tex <==
58.4


==> stats/e2_exploratory/means/social_info_green/social_resampling/blue_bias/proportion.tex <==
0.584


==> stats/e2_exploratory/means/social_info_green/social_resampling/green_bias/percentage.tex <==
60


==> stats/e2_exploratory/means/social_info_green/social_resampling/green_bias/proportion.tex <==
0.6


==> stats/e2_exploratory/tests/soc_info_accuracy/soc_resampling-soc_bias/prereg.tex <==
$\chi^2(1)=32.62$, $p<0.001$


==> stats/e2_exploratory/tests/soc_info_bias/soc_resampling-soc_bias/prereg.tex <==
$\chi^2(1)=293.27$, $p<0.001$


==> stats/e2_exploratory/tests/soc_info_green/blue_bias/soc_resampling-soc_bias/prereg.tex <==
$\chi^2(1)=183.08$, $p<0.001$


==> stats/e2_exploratory/tests/soc_info_green/green_bias/soc_bias-soc_resampling/prereg.tex <==
hi


==> stats/e2_perceptual_priming/summaries/chose_green/percentage.tex <==
53.4


==> stats/e2_perceptual_priming/summaries/green_shown=FALSE/chose_green/percentage.tex <==
53.5


==> stats/e2_perceptual_priming/summaries/green_shown=FALSE/n.tex <==
1,891


==> stats/e2_perceptual_priming/summaries/green_shown=TRUE/chose_green/percentage.tex <==
53.3


==> stats/e2_perceptual_priming/summaries/green_shown=TRUE/n.tex <==
1,867


==> stats/e2_perceptual_priming/summaries/randomization_color=blue/chose_green/percentage.tex <==
50


==> stats/e2_perceptual_priming/summaries/randomization_color=blue/n.tex <==
1,911


==> stats/e2_perceptual_priming/summaries/randomization_color=green/chose_green/percentage.tex <==
56.9


==> stats/e2_perceptual_priming/summaries/randomization_color=green/n.tex <==
1,847


==> stats/simulations/asocial/absolute_bias/lower_ci.tex <==
0.204


==> stats/simulations/asocial/absolute_bias/mean.tex <==
0.258


==> stats/simulations/asocial/absolute_bias/upper_ci.tex <==
0.315


==> stats/simulations/asocial/bias_standard_deviation/lower_ci.tex <==
0.006


==> stats/simulations/asocial/bias_standard_deviation/mean.tex <==
0.053


==> stats/simulations/asocial/bias_standard_deviation/upper_ci.tex <==
0.172


==> stats/simulations/asocial/green_dots_48/lower_ci.tex <==
-16.714


==> stats/simulations/asocial/green_dots_48/mean.tex <==
0.137


==> stats/simulations/asocial/green_dots_48/upper_ci.tex <==
17.334


==> stats/simulations/asocial/green_dots_49/lower_ci.tex <==
-16.435


==> stats/simulations/asocial/green_dots_49/mean.tex <==
0.347


==> stats/simulations/asocial/green_dots_49/upper_ci.tex <==
17.501


==> stats/simulations/asocial/green_dots_51/lower_ci.tex <==
-15.853


==> stats/simulations/asocial/green_dots_51/mean.tex <==
0.993


==> stats/simulations/asocial/green_dots_51/upper_ci.tex <==
18.199


==> stats/simulations/asocial/green_dots_52/lower_ci.tex <==
-15.525


==> stats/simulations/asocial/green_dots_52/mean.tex <==
1.286


==> stats/simulations/asocial/green_dots_52/upper_ci.tex <==
18.497


==> stats/simulations/asocial/intercept/lower_ci.tex <==
-17.777


==> stats/simulations/asocial/intercept/mean.tex <==
-0.583


==> stats/simulations/asocial/intercept/upper_ci.tex <==
16.236


==> stats/simulations/asocial/n.tex <==
10,000


==> stats/simulations/social/absolute_bias/lower_ci.tex <==
0.29


==> stats/simulations/social/absolute_bias/mean.tex <==
0.37


==> stats/simulations/social/absolute_bias/upper_ci.tex <==
0.451


==> stats/simulations/social/bias_standard_deviation/lower_ci.tex <==
0.338


==> stats/simulations/social/bias_standard_deviation/mean.tex <==
0.468


==> stats/simulations/social/bias_standard_deviation/upper_ci.tex <==
0.585


==> stats/simulations/social/green_dots_48/lower_ci.tex <==
-18.816


==> stats/simulations/social/green_dots_48/mean.tex <==
-0.968


==> stats/simulations/social/green_dots_48/upper_ci.tex <==
16.481


==> stats/simulations/social/green_dots_49/lower_ci.tex <==
-18.452


==> stats/simulations/social/green_dots_49/mean.tex <==
-0.629


==> stats/simulations/social/green_dots_49/upper_ci.tex <==
16.77


==> stats/simulations/social/green_dots_51/lower_ci.tex <==
-17.746


==> stats/simulations/social/green_dots_51/mean.tex <==
0.028


==> stats/simulations/social/green_dots_51/upper_ci.tex <==
17.445


==> stats/simulations/social/green_dots_52/lower_ci.tex <==
-17.716


==> stats/simulations/social/green_dots_52/mean.tex <==
0.122


==> stats/simulations/social/green_dots_52/upper_ci.tex <==
17.539


==> stats/simulations/social/intercept/lower_ci.tex <==
-17.814


==> stats/simulations/social/intercept/mean.tex <==
-0.444


==> stats/simulations/social/intercept/upper_ci.tex <==
17.386


==> stats/simulations/social/n.tex <==
10,000


==> stats/simulations/social/vote_coefficient/lower_ci.tex <==
0.193


==> stats/simulations/social/vote_coefficient/mean.tex <==
0.233


==> stats/simulations/social/vote_coefficient/upper_ci.tex <==
0.274


==> tables/e1/row1.tex <==
& & \multicolumn{2}{c}{\textbf{Asocial / Control}} \\
& & Reported & Prereg 
\\

==> tables/e1/row2.tex <==
\multirow{2}{*}{\textbf{\shortstack{Asocial / \\ Motivated}}} 
& Bias & 
\input{stats/e1/table_stats/chose_bias/aso_control-aso_bias/reported} & 
\input{stats/e1/table_stats/chose_bias/aso_control-aso_bias/prereg} & 
\multicolumn{2}{c}{\textbf{Asocial / Motivated}} & 
\\ 
& Accuracy & 
\input{stats/e1/table_stats/chose_correct/aso_control-aso_bias/reported} &
\input{stats/e1/table_stats/chose_correct/aso_control-aso_bias/prereg} &
Reported & Prereg &
\\

==> tables/e1/row3.tex <==
\multirow{2}{*}{\textbf{\shortstack{Social / \\ Control}}} 
& Bias & 
\input{stats/e1/table_stats/chose_bias/aso_control-soc_control/reported} & 
\input{stats/e1/table_stats/chose_bias/aso_control-soc_control/prereg} & 
\input{stats/e1/table_stats/chose_bias/aso_bias-soc_control/reported} & 
\input{stats/e1/table_stats/chose_bias/aso_bias-soc_control/prereg} & 
\multicolumn{2}{c}{\textbf{Social / Control}} & 
\\ 
& Accuracy & 
\input{stats/e1/table_stats/chose_correct/aso_control-soc_control/reported} & 
\input{stats/e1/table_stats/chose_correct/aso_control-soc_control/prereg} & 
\input{stats/e1/table_stats/chose_correct/aso_bias-soc_control/reported} & 
\input{stats/e1/table_stats/chose_correct/aso_bias-soc_control/prereg} & 
Reported & Prereg &
\\

==> tables/e1/row4.tex <==
\multirow{2}{*}{\textbf{\shortstack{Social / \\ Motivated}}} 
& Bias & 
\input{stats/e1/table_stats/chose_bias/aso_control-soc_bias/reported} & 
\input{stats/e1/table_stats/chose_bias/aso_control-soc_bias/prereg} & 
\input{stats/e1/table_stats/chose_bias/aso_bias-soc_bias/reported} & 
\input{stats/e1/table_stats/chose_bias/aso_bias-soc_bias/prereg} & 
\input{stats/e1/table_stats/chose_bias/soc_bias-soc_control/reported} & 
\input{stats/e1/table_stats/chose_bias/soc_bias-soc_control/prereg} & 
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Social / Motivated}}}
\\ 
& Accuracy & 
\input{stats/e1/table_stats/chose_correct/aso_control-soc_bias/reported} & 
\input{stats/e1/table_stats/chose_correct/aso_control-soc_bias/prereg} & 
\input{stats/e1/table_stats/chose_correct/aso_bias-soc_bias/reported} & 
\input{stats/e1/table_stats/chose_correct/aso_bias-soc_bias/prereg} & 
\input{stats/e1/table_stats/chose_correct/soc_bias-soc_control/reported} &
\input{stats/e1/table_stats/chose_correct/soc_bias-soc_control/prereg} & 
\\

==> tables/e2/row1.tex <==
& & \multicolumn{2}{c}{\textbf{Asocial / Motivated}} \\
& & Reported & Pre-reg 
\\

==> tables/e2/row2.tex <==
\multirow{2}{*}{\textbf{\shortstack{Social / \\ Motivated}}} 
& Bias & 
\input{stats/e2/table_stats/chose_bias/aso_bias-soc_bias/reported} & 
\input{stats/e2/table_stats/chose_bias/aso_bias-soc_bias/prereg} & 
\multicolumn{2}{c}{\textbf{Social / Motivated}} & 
\\ 
& Accuracy & 
\input{stats/e2/table_stats/chose_correct/aso_bias-soc_bias/reported} &
\input{stats/e2/table_stats/chose_correct/aso_bias-soc_bias/prereg} &
Reported & Pre-reg &
\\

==> tables/e2/row3.tex <==
\multirow{2}{*}{\textbf{\shortstack{Social / \\ Resampling}}} 
& Bias & 
\input{stats/e2/table_stats/chose_bias/aso_bias-soc_resampling/reported} & 
\input{stats/e2/table_stats/chose_bias/aso_bias-soc_resampling/prereg} & 
\input{stats/e2/table_stats/chose_bias/soc_resampling-soc_bias/reported} & 
\input{stats/e2/table_stats/chose_bias/soc_resampling-soc_bias/prereg} & 
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Social / Resampling}}}
\\ 
& Accuracy & 
\input{stats/e2/table_stats/chose_correct/aso_bias-soc_resampling/reported} & 
\input{stats/e2/table_stats/chose_correct/aso_bias-soc_resampling/prereg} & 
\input{stats/e2/table_stats/chose_correct/soc_resampling-soc_bias/reported} &
\input{stats/e2/table_stats/chose_correct/soc_resampling-soc_bias/prereg} & 
\\
